Invisible Perturbations: Physical Adversarial Examples Exploiting the Rolling Shutter Effect

Physical adversarial examples for camera-based computer vision have so far been achieved through visible artifacts -- a sticker on a Stop sign, colorful borders around eyeglasses or a 3D printed object with a colorful texture. An implicit assumption here is that the perturbations must be visible so that a camera can sense them. By contrast, we contribute a procedure to generate, for the first time, physical adversarial examples that are invisible to human eyes. Rather than modifying the victim object with visible artifacts, we modify light that illuminates the object. We demonstrate how an attacker can craft a modulated light signal that adversarially illuminates a scene and causes targeted misclassifications on a state-of-the-art ImageNet deep learning model. Concretely, we exploit the radiometric rolling shutter effect in commodity cameras to create precise striping patterns that appear on images. To human eyes, it appears like the object is illuminated, but the camera creates an image with stripes that will cause ML models to output the attacker-desired classification. We conduct a range of simulation and physical experiments with LEDs, demonstrating targeted attack rates up to 84%.

==> defense.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Potential Defenses against The Attack}\label{sec:defense}

\begin{enumerate}
\item  Processing the captured image by changing brightness/contrast might reduce the attack efficacy
\item Using video and then merge photos of multiple instance?
\item Merge photos of multiple cameras (assuming they are of different model with different $T_r$, etc.)
\item 
\end{enumerate}

==> images/rs.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
  % uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

  % Shape: Axis 2D [id:dp04502427511754847]
  \draw  (70.5,138) -- (554.5,138)(70.5,14) -- (70.5,138) -- cycle (547.5,133) -- (554.5,138) -- (547.5,143) (65.5,21) -- (70.5,14) -- (75.5,21) (90.5,133) -- (90.5,143)(110.5,133) -- (110.5,143)(130.5,133) -- (130.5,143)(150.5,133) -- (150.5,143)(170.5,133) -- (170.5,143)(190.5,133) -- (190.5,143)(210.5,133) -- (210.5,143)(230.5,133) -- (230.5,143)(250.5,133) -- (250.5,143)(270.5,133) -- (270.5,143)(290.5,133) -- (290.5,143)(310.5,133) -- (310.5,143)(330.5,133) -- (330.5,143)(350.5,133) -- (350.5,143)(370.5,133) -- (370.5,143)(390.5,133) -- (390.5,143)(410.5,133) -- (410.5,143)(430.5,133) -- (430.5,143)(450.5,133) -- (450.5,143)(470.5,133) -- (470.5,143)(490.5,133) -- (490.5,143)(510.5,133) -- (510.5,143)(530.5,133) -- (530.5,143)(65.5,118) -- (75.5,118)(65.5,98) -- (75.5,98)(65.5,78) -- (75.5,78)(65.5,58) -- (75.5,58)(65.5,38) -- (75.5,38) ;
  \draw   ;
  % Shape: Axis 2D [id:dp9636794177818229]
  \draw  (70.5,278) -- (554.5,278)(70.5,154) -- (70.5,278) -- cycle (547.5,273) -- (554.5,278) -- (547.5,283) (65.5,161) -- (70.5,154) -- (75.5,161)  ;
  % Shape: Right Angle [id:dp9200019591904323]
  \draw   (84,62) -- (124.49,62) -- (124.49,116) ;
  % Shape: Right Angle [id:dp14796249745369527]
  \draw   (124.49,116) -- (165.18,116.38) -- (165.36,62.38) ;
  % Shape: Right Angle [id:dp7259516581862786]
  \draw   (165.57,63) -- (206.06,63) -- (206.06,117) ;
  % Shape: Right Angle [id:dp02520352346544885]
  \draw   (206.06,117) -- (246.75,117.38) -- (246.93,63.38) ;
  % Shape: Right Angle [id:dp44815194196292407]
  \draw   (246.54,64) -- (287.03,64) -- (287.03,118) ;
  % Shape: Right Angle [id:dp6730587264050962]
  \draw   (287.63,117) -- (328.32,117.38) -- (328.5,63.38) ;
  % Shape: Rectangle [id:dp2792247565829662]
  \draw   (90,173.47) -- (180.5,173.47) -- (180.5,187.79) -- (90,187.79) -- cycle ;
  % Shape: Rectangle [id:dp8043521623831285]
  \draw   (102,187.79) -- (192.5,187.79) -- (192.5,202.11) -- (102,202.11) -- cycle ;
  % Shape: Rectangle [id:dp9152972660886962]
  \draw   (111,202.11) -- (201.5,202.11) -- (201.5,216.43) -- (111,216.43) -- cycle ;
  % Shape: Rectangle [id:dp23241449910886214]
  \draw   (123,216.43) -- (213.5,216.43) -- (213.5,230.75) -- (123,230.75) -- cycle ;
  % Shape: Rectangle [id:dp0739413357225065]
  \draw   (238,250.04) -- (328.5,250.04) -- (328.5,262.52) -- (238,262.52) -- cycle ;
  % Shape: Rectangle [id:dp33100671564064]
  \draw   (250,262.52) -- (340.5,262.52) -- (340.5,275) -- (250,275) -- cycle ;
  % Shape: Rectangle [id:dp11793986217928332]
  \draw   (169.5,174.12) -- (180.5,174.12) -- (180.5,188.44) -- (169.5,188.44) -- cycle ;

  % Text Node
  \draw (170,174.45) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle t_{r}$};
  % Text Node
  \draw (124,174.44) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle t_{e}$};
  % Text Node
  \draw (181,188.45) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle t_{r}$};
  % Text Node
  \draw (135,188.44) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle t_{e}$};
  % Text Node
  \draw (190,202.45) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle t_{r}$};
  % Text Node
  \draw (144,202.44) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle t_{e}$};


\end{tikzpicture}

